Do As I Can, Not As I Say: Grounding Language in Robotic Affordances

Large language models can encode a wealth of semantic knowledge about the world. Such knowledge could be extremely useful to robots aiming to act upon high-level, temporally extended instructions expressed in natural language. However, a significant weakness of language models is that they lack real-world experience, which makes it difficult to leverage them for decision making within a given embodiment. For example, asking a language model to describe how to clean a spill might result in a reasonable narrative, but it may not be applicable to a particular agent, such as a robot, that needs to perform this task in a particular environment. We propose to provide real-world grounding by means of pretrained skills, which are used to constrain the model to propose natural language actions that are both feasible and contextually appropriate. The robot can act as the language model's "hands and eyes," while the language model supplies high-level semantic knowledge about the task. We show how low-level skills can be combined with large language models so that the language model provides high-level knowledge about the procedures for performing complex and temporally-extended instructions, while value functions associated with these skills provide the grounding necessary to connect this knowledge to a particular physical environment. We evaluate our method on a number of real-world robotic tasks, where we show the need for real-world grounding and that this approach is capable of completing long-horizon, abstract, natural language instructions on a mobile manipulator. The project's website and the video can be found at https://say-can.github.io/.

==> all_tasks.tex <==

\begin{table}[htb]
\ContinuedFloat
\rowcolors{3}{white}{lightgray}
\small
\begin{center}
\renewcommand{\arraystretch}{1.2}
\begin{subfigure}[b]{1.0\textwidth}
         \centering
\begin{tabular}{|p{0.5\textwidth}| p{0.05\textwidth}p{0.1\textwidth}|p{0.05\textwidth}p{0.1\textwidth}|}
\hhline{~----}
\multicolumn{1}{c}{} & \multicolumn{2}{ |c|}{Mock Kitchen}  & \multicolumn{2}{| c |}{ Kitchen} \\
\hline
\textbf{Instruction}  & \textbf{Plan} & \textbf{Execution}  & \textbf{Plan} & \textbf{Execution} \\ \hline\hline
How would you pick up the coke can & 1 & 1 & 1 & 1 \\
How would you put the coke can in the your gripper & 0 & 0 & 0 & 0 \\
How would you grasp the coke can & 1 & 1 & 1 & 1 \\
How would you hold onto the coke can & 1 & 1 & 1 & 1 \\
How would you lift and hold the coke can up & 0 &  0& 0 & 0 \\
How would you put the coke can down & 1 & 1 & 1 & 1 \\
How would you place the coke can on the table & 1 & 1 &  1 & 1\\
How would you let go of the coke can & 0 & 0 & 1 & 1\\
How would you release the coke can & 0 & 0 & 1 & 1\\
How would you place the coke can & 0 & 0 & 1 & 1 \\
How would you move to the table & 1 & 1 & 1 & 1 \\
How would you go to the table & 1 & 1 & 1 & 1 \\
How would you park at the table & 1 & 1 & 1 & 1 \\
How would you come to the table & 1 & 1 & 1 & 1 \\
How would you navigate to the table & 1 & 1 & 1 & 1 \\
\hline
\end{tabular}
\caption{NL Single Primitive}
\end{subfigure}
\end{center}
\end{table}

\begin{table}[htb]
\ContinuedFloat
\begin{center}
\rowcolors{3}{white}{lightgray}
\begin{subfigure}[b]{1.0\textwidth}
         \centering
         
\begin{tabular}{|p{0.5\textwidth}| p{0.05\textwidth}p{0.1\textwidth}|p{0.05\textwidth}p{0.1\textwidth}|}
\hhline{~----}
\multicolumn{1}{c}{} & \multicolumn{2}{ |c|}{Mock Kitchen}  & \multicolumn{2}{| c |}{ Kitchen} \\
\hline
\textbf{Instruction}  & \textbf{Plan} & \textbf{Execution}  & \textbf{Plan} & \textbf{Execution} \\ \hline\hline
How would you throw away the apple &  1 & 1 & 1 & 0\\
How would you bring me a sponge? & 1 & 1 & 1 & 1 \\
How would you bring me a coke can & 1 & 1 & 1 & 1\\
How would you grab me an apple & 1 & 1 & - & -\\
How would you grab me a 7up from the table & 1 & 1 & - & -\\
How would you deliver the red bull to the close counter & 1 & 0 & - & -\\
How would you throw away the jalapeno chips & 1 & 1 & - & -\\
How would you restock the rice chips on the far counter & 1 & 1 & 1 & 1 \\
How would you recycle the coke can & 0 & 0 & - &  -\\
How would you throw away the water bottle & 1 & 1 & 1 & 1\\
How would you bring me something hydrating & 1 & 1 & - & -\\
How would you put the apple back on the far counter & 1 & 1 & - & -\\
How would you recycle the 7up & 0 & 0 & 0 & 0\\
How would you throw away jalapeno chips & 0 & 0 & - & -\\
How would you compost the apple & 1 & 0 & - & -\\
\hline
\end{tabular}
\caption{NL Verb}
\end{subfigure}
\end{center}
\end{table}

\begin{table}
\small
\rowcolors{3}{white}{lightgray}

\ContinuedFloat
\begin{center}
\begin{subfigure}[b]{1.0\textwidth}
         \centering
\begin{tabular}{|p{0.5\textwidth}| p{0.05\textwidth}p{0.1\textwidth}|p{0.05\textwidth}p{0.1\textwidth}|}
\hhline{~----}
\multicolumn{1}{c}{} & \multicolumn{2}{ |c|}{Mock Kitchen}  & \multicolumn{2}{| c |}{ Kitchen} \\
\hline
\textbf{Instruction}  & \textbf{Plan} & \textbf{Execution}  & \textbf{Plan} & \textbf{Execution} \\ \hline\hline
How would you bring me lime drink & 1 & 1 & 1 & 1 \\
How would you bring me something to clean the kitchen with & 1 & 1 & 0 & 0 \\
How would you bring me something to eat & 1 & 1 & - & - \\
How would you put the grapefruit drink on the close counter & 0 & 0 & - &-\\
How would you move the sugary drink to the far counter & 0 & 0 &- &- \\
How would you move something with caffine from the table to the close counter & 0 & 0 &- &- \\
How would you bring me an energy bar & 1 & 1  &- &-\\
How would you bring me something to quench my thirst & 1 & 1 & 1 &1 \\
How would you bring me a fruit & 1 & 0 & 1 & 1 \\
How would you bring me a fruit from the close counter & 1 & 1 & - & - \\
How would you bring me something that is not a fruit from the close counter & 0 & 0 & - & -\\
How would you bring me a soda from the table & 0 & 0 & 0 & 0 \\
How would you bring me a soda & 1 & 1 & 1 & 1  \\
How would you bring me a bag of chips from close counter & 0 & 0 & 0 & 0 \\
How would you bring me a snack & 1 & 1 & 1 & 0 \\

\hline
\end{tabular}
\caption{NL Nouns}
\end{subfigure}
\end{center}
\end{table}

\begin{table}[htb]
\ContinuedFloat
\begin{center}
\rowcolors{3}{white}{lightgray}
\begin{subfigure}[b]{1.0\textwidth}
         \centering
\begin{tabular}{|p{0.5\textwidth}| p{0.05\textwidth}p{0.1\textwidth}|p{0.05\textwidth}p{0.1\textwidth}|}
\hhline{~----}
\multicolumn{1}{c}{} & \multicolumn{2}{ |c|}{Mock Kitchen}  & \multicolumn{2}{| c |}{ Kitchen} \\
\hline
\textbf{Instruction}  & \textbf{Plan} & \textbf{Execution}  & \textbf{Plan} & \textbf{Execution} \\ \hline\hline
How would you pick up the apple and move it to the trash & 1 & 0 & 1 & 0 \\
How would you pick up the sponge and bring it to me & 1 & 1 & 1 & 1 \\
How would you pick up the coke can and bring it to me & 1 & 1 & 1 & 1 \\
How would you pick up the apple and bring it to me & 1 & 1 & - & - \\
How would you pick up the 7up and bring it to me & 1 & 1 & - &- \\
How would you pick up the redbull and move it to the close counter & 1 & 0 &- &-\\
How would you pick up the jalapeno chips and move it to the trash & 1 & 1 & -&-\\
How would you pick up the rice chips and move it to the far counter & 1 & 1 & 1 & 0 \\
How would you pick up the coke can and move it to the trash & 1 & 1 & - & - \\
How would you pick up the water bottle and move it to the trash & 1 & 1 & 1 & 1 \\
How would you pick up the grapefruit soda and bring it to me & 1 & 1 & - & - \\
How would you pick up the apple and move it to the far counter & 1 & 1 & - & -\\
How would you pick up the 7up and move it to the trash & 1 & 1 & 0 & 0 \\
How would you pick up the jalepeno chips and move it to the trash & 1 & 1 & - & - \\
How would you pick up the apple and move it to the trash & 1 & 1 & - & - \\

\hline
\end{tabular}
\caption{Structured Language}
\end{subfigure}
\end{center}
\end{table}

\begin{table}
\small
\ContinuedFloat
\begin{center}
\rowcolors{3}{white}{lightgray}
\begin{subfigure}[b]{1.0\textwidth}
         \centering
\begin{tabular}{|p{0.5\textwidth}| p{0.05\textwidth}p{0.1\textwidth}|p{0.05\textwidth}p{0.1\textwidth}|}
\hhline{~----}
\multicolumn{1}{c}{} & \multicolumn{2}{ |c|}{Mock Kitchen}  & \multicolumn{2}{| c |}{ Kitchen} \\
\hline
\textbf{Instruction}  & \textbf{Plan} & \textbf{Execution}  & \textbf{Plan} & \textbf{Execution} \\ \hline\hline
How would you put the coke can down on the far counter(with operator) & 1 & 1 & - & - \\
How would you put the coke can down on the far counter(at table) & 1 & 0 & - & - \\
How would you put the coke can down on the far counter(at table with coke can in hand) &  1 & 1 &- & - \\
How would you put the coke can down on the far counter(at far counter with coke can in hand) &  1 & 1 &- & - \\

How would you put the sponge on the close counter(with operator) & 1 & 1 & - & - \\
How would you put the sponge on the close counter(at far counter) & 1 & 1 & - & - \\
How would you put the sponge on the close counter(at far counter with sponge in hand) &  0 & 0 &- & - \\
How would you put the sponge on the close counter(at close counter with coke can in hand) &  0 & 0 &- & - \\
How would you pick up the drink from the far counter & 1 & 1 & - & - \\
I left something on the table, can you throw it away? &  0 & 0 &- & - \\
I left something on the table or the counter, can you bring it to me?  &  0 & 0 &- & - \\
\hline
\end{tabular}
\caption{Embodiment}
\end{subfigure}
\end{center}
\end{table}

\begin{table}[htb]
\ContinuedFloat
\begin{center}
\rowcolors{3}{white}{lightgray}
\begin{subfigure}[b]{1.0\textwidth}
         \centering
\begin{tabular}{|p{0.5\textwidth}| p{0.05\textwidth}p{0.1\textwidth}|p{0.05\textwidth}p{0.1\textwidth}|}
\hhline{~----}
\multicolumn{1}{c}{} & \multicolumn{2}{ |c|}{Mock Kitchen}  & \multicolumn{2}{| c |}{ Kitchen} \\
\hline
\textbf{Instruction}  & \textbf{Plan} & \textbf{Execution}  & \textbf{Plan} & \textbf{Execution} \\ \hline\hline
I opened a pepsi earlier. How would you bring me an open can? & 1 & 1 & - & - \\
I spilled my coke, can you bring me a replacement? & 1 & 1 & 1 & 1 \\
I spilled my coke, can you bring me something to clean it up? &1  & 1 & 1 & 1 \\
I accidentally dropped that jalapeno chip bag after eating it. Would you mind throwing it away? & 0 & 0 & - & - \\
I like fruits, can you bring me something I'd like? & 1 & 1 &- &-\\
There is a close counter, far counter, and table. How would you visit all the locations? & 1 & 1 &- &-\\
There is a close counter, trash can, and table. How would you visit all the locations? & 1 &1 &- & -\\
Redbull is my favorite drink, can I have one please? & 1 & 1 & 1&1 \\
Would you bring me a coke can? & 1 & 1 & 1 & 1\\
Please, move the pepsi to the close counter & 1 &  1 & - & -\\
Please, move the ppsi(intentional typo) to the close cuonter & 0 & 0 & - & -\\
Can you move the coke can to the far counter? & 1 & 1 & - & - \\
Can you move coke can to far counter? & 1 & 0 & - & - \\
Would you throw away the bag of chips for me? & 0 & 0 & 0 & 0 \\
Would you throw away the bag of chpis(intentional typo) for me? & 0 & 0 & - & - \\
\hline
\end{tabular}
\caption{Crowd-Sourced}
\end{subfigure}

\end{center}
\end{table}

\begin{table}
\small
\ContinuedFloat
\begin{center}
\rowcolors{3}{white}{lightgray}
\begin{subfigure}[b]{1.0\textwidth}
         \centering
\begin{tabular}{|p{0.5\textwidth}| p{0.05\textwidth}p{0.1\textwidth}|p{0.05\textwidth}p{0.1\textwidth}|}
\hhline{~----}
\multicolumn{1}{c}{} & \multicolumn{2}{ |c|}{Mock Kitchen}  & \multicolumn{2}{| c |}{ Kitchen} \\
\hline
\textbf{Instruction}  & \textbf{Plan} & \textbf{Execution}  & \textbf{Plan} & \textbf{Execution} \\ \hline\hline
How would you put an energy bar and water bottle on the table & 0 & 0 & 0 & 0 \\
How would you bring me a lime soda and a bag of chips & 0 & 0 & 0 & 0 \\
Can you throw away the apple and bring me a coke & 1 & 1 & - & - \\
How would you bring me a 7up can and a tea? & 0 & 0 &- &- \\
How would throw away all the items on the table? & 0 & 0 & 0 & 0 \\
How would you move an multigrain chips to the table and an apple to the far counter? & 1 & 1 &- &- \\
How would you move the lime soda, the sponge, and the water bottle to the table? & 1 & 0 &- &- \\
How would you bring me two sodas? & 0 & 0 & - & - \\
How would you move three cokes to the trash can? & 0 & 0 & - & -\\
How would you throw away two cokes? & 1 & 1 & 1 & 1 \\
How would you bring me two different sodas? & 1 &  1 & - & -\\
How would you bring me an apple, a coke, and water bottle? & 1 & 0 & - & - \\
I spilled my coke on the table, how would you throw it away and then bring me something to help clean? & 1 & 1 & 1 & 1 \\
I just worked out, can you bring me a drink and a snack to recover? & 0 & 0 & - & -\\
How would you bring me a fruit, a soda, and a bag of chips for lunch & 0 & 0 & 0 & 0\\

\hline
\end{tabular}
\caption{Long-Horizon}
\end{subfigure}


\caption{\textbf{List of all instruction and experiment results} We evaluate the algorithm on 101 instructions on 2 scenes, 147 experiments in total. The metrics and success definitions can be found in Sec.~\ref{sec:metrics}. A 0 indicates failure, 1 indicates success, and - indicates the experiment was not ran in the particular setup.}
\label{tab:all_results}
\end{center}
\end{table}


==> short_conclusion.tex <==

\section{Conclusions and Limitations}

We presented \algname, a method that enables leveraging and grounding the rich knowledge in large language models to complete embodied tasks.
For real-world grounding, we use RL-based value functions for the individual skills that provide affordances of what is possible in the world, and use textual labels for these skills as potential responses that are scored by a language model.
We evaluated this approach on a number of real-world robotic tasks that involve a mobile manipulator robot accomplishing a large set of long-horizon natural language instructions in a real kitchen.




While \algname presents a viable way to ground language models in agents' affordances, it has a number of limitations.
First, we expect this method to inherit the limitations and biases of LLMs~\citep{bender2021dangers,bommasani2021opportunities},
including the dependence on the training data.
In addition, we observe that even though \algname allows the users to interact with the agents using natural language commands, the primary bottleneck of the system is in the range and capabilities of the underlying skills.
To illustrate this, we present representative failure cases in Appendix~\ref{sec:app_exp}.











